Seculator: A Fast and Secure Neural Processing Unit

Securing deep neural networks (DNNs) is a problem of significant interest since an ML model incorporates high-quality intellectual property, features of data sets painstakingly collated by mechanical turks, and novel methods of training on large cluster computers. Sadly, attacks to extract model parameters are on the rise, and thus designers are being forced to create architectures for securing such models. State-of-the-art proposals in this field take the deterministic memory access patterns of such networks into cognizance (albeit partially), group a set of memory blocks into a tile, and maintain state at the level of tiles (to reduce storage space). For providing integrity guarantees (tamper avoidance), they don't propose any significant optimizations, and still maintain block-level state. We observe that it is possible to exploit the deterministic memory access patterns of DNNs even further, and maintain state information for only the current tile and current layer, which may comprise a large number of tiles. This reduces the storage space, reduces the number of memory accesses, increases performance, and simplifies the design without sacrificing any security guarantees. The key techniques in our proposed accelerator architecture, Seculator, are to encode memory access patterns to create a small HW-based tile version number generator for a given layer, and to store layer-level MACs. We completely eliminate the need for having a MAC cache and a tile version number store (as used in related work). We show that using intelligently-designed mathematical operations, these structures are not required. By reducing such overheads, we show a speedup of 16% over the closest competing work.

==> CipherCharacterization.tex <==
\subsubsection{Cipher Characterization}
In order to estimate the amount of energy overhead of the AES cipher. The AES implementation from the OpenSSH library is characterized using Tejas. Table \ref{tab:config} presents the Tejas system configuration and Table \ref{tab:cipher_results} presents the results.
The results for the simulation of the ciphers are presented as:
\begin{table}[!h]
\begin{center}
\begin{tabular}{ |c | c | c| }
\hline
\textbf{Parameters} & \textbf{AES} & \textbf{RC4}\\
\hline
IPC(microOps) & 0.2413 & 0.6807\\
Cycles & 203901 & -\\
L1 Hit Rate & 0.88 & -\\
L2 Hit Rate & 0.66 & -\\
Total energy & 177956.5837 & 0 \\

\hline
\end{tabular}
\caption{\label{tab:cipher_results} Results after simulating OpenSSH cipher on Tejas.}

\end{center}
\end{table}

\begin{table}[!h]
\begin{center}
\begin{tabular}{ |c |c || c | c| }
\hline
\textbf{Parameter} & \textbf{Value}  & \textbf{L1} & \textbf{Values}\\
\hline
 Cores & 1 & Block Size & 64 bytes  \\ 
 Issue Width & 4 & Associativity & 8\\  
 Pipeline Type & out-of-order & Size & 32KB\\
  Frequency & 3.2 GHz  & Latency & 4 Cycles \\
 \hline
 \hline
 \multicolumn{2}{|c|}{\textbf{L2 Cache (Shared)}}\\
 \cline{1-2}
 Block Size & 64 Bytes \\
 Associativity & 8 \\
 Bank Size & 256 KB\\
 Banks & 8\\
 Latency & 8 cycles\\
 Write Mode & Write through \\
 \cline{1-2}
\end{tabular}
\caption{\label{tab:config} Tejas Configuration.}
\end{center}
\end{table}

==> Contribution.tex <==
\section{Contribution}
We will be focusing on answering the following questions:
\begin{enumerate}
    \item What is the impact of model compression on the CNN's accuracy.
\end{enumerate}

==> MatMul.tex <==

\subsection{Matrix Multiplication (MatMul)}
We analyze the data access pattern in the case of MatMuls as it is extensively used in several ML workloads including transformers \cite{transformer}. We tile the input matrices $A$ and $B$ as shown in Figure \ref{fig:matrix}. The tile size for matrix A is $H' \times C'$ and the matrix B is $C' \times W'$ will generate output tile size of $H' \times W'$. We note that $C' < C$  will lead to a partially computed tile of size $H' \times W'$. Additional $C/C'$ computations will be required to generate the final tile. We term these additional iterations as the \textit{sample height}. 
We analyze the following tiling scenarios and present our findings in Table \ref{tab:dataflow_matrix}:

%\begin{enumerate}[leftmargin=.5cm]
    \circlenew{1} \textit{Partial matrix-loading:} The scheduling scheme is sub-classified into three categories where we anchor one of the three entities involved in the computation: Matrix $A$, $B$ or the output. We respect the rules of matrix computation while analyzing the data access pattern. In the \textit{anchored $A$} scheme, matrix $B$ can only move across the column direction, generating $W/W'$ partially computed output tiles of size $H' \times W'$. The number of output tiles generated per tile of matrix $A$ is the \textit{sample point}. All the tiles will have the same version number.
    
     Next, the tile of matrix $A$ moves along the column direction, while, the tile of matrix $B$ is scheduled to iterate along the columns of the consecutive row. The previously generated output tiles are updated. The process repeats for $C/C'$ times. In the next step, the tile of matrix $A$ moves to the consecutive row and the whole process repeats itself for $H/H'$ times generating an identical pattern. We term this as the \textit{sample count}. The \textit{anchored B} scheme is just a reverse of the previous method, where we fix matrix $B$, and the corresponding tiles of matrix $A$ is fetched from the memory.
    
   % Similarly, for \textit{anchored $B$}, the tile of matrix $B$ will be fixed and tile $A$ will iterate along the row direction generating $P/P'$ partially computed output tiles of dimension $P' \times K'$. The number of output tiles generated per tile of matrix $B$ is the \textit{sample count}. After all the rows of tile $A$ are covered, tile $B$ will move in the row direction, while, the tile of $A$ will be scheduled to iterate along all the rows of the consecutive column. The generated output tiles will be updated for $C/C'$ times. Next, the tile $B$ will move to the consecutive column and the whole process will repeat itself for $K/K'$ iterations.
   In the \textit{anchored output}, the output tile of size $H' \times W'$ is fixed. The input tile of matrix $A$ of size $H' \times C'$ and $B$ of size $C' \times W'$ are fetched from the memory to compute the output. The process repeats for $C/C'$ times, with each update the VN is incremented. Then we move to the next output tile. This process generates a repeated linear pattern.
    
    \circlenew{2} \textit{Row-major loading:}  In this scenario, the scheduling of tiles for matrix $A$ and $B$ will be completely synchronized. Tile of matrix $A$ moves along the row while the tile of matrix $B$ moves along the column. All the elements required to generate a output tile are available in the TCB.  No storage of the partially computed output will be required leading to a straight line pattern.
  \circlenew{3} \textit{No tiling:} The whole computation is done in a single iteration. No pattern will be generated. 
%\end{enumerate}

%\begin{figure}[h]
%    \centering
%    \includegraphics[scale=0.6]{Figures/matrix.pdf}
%    \caption{An illustration of matrix multiplication. The output tile size is constrained by the value of the input matrix tile size.}
%    \label{fig:matrix}
%\end{figure}



%\subsubsection{Matrix-Vector Multiplication} The matrix multiplication is special case of matrix multiplication, where, we view vector as the column matrix B. In this case, the value of $K$ will always be 1. The output matrix will be a column matrix of dimension $(P\times1)$



%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%MATRIX
\begin{scriptsize}
\begin{table}[!h]
\begin{center}
\begin{tabular}{ |p{0.1\linewidth}|p{0.3\linewidth}|p{0.2\linewidth}|p{0.2\linewidth}|} 
\hline
\rowcolor{gray!20}
\textbf{Tiling Style}  & \textbf{Representation} & \textbf{Sample pt; Ht.; Count}  & \textbf{Pattern}\\
%\rowcolor{gray!20}
 %\textbf{K$\neq$1}
 \hline

\rowcolor{blue!10}
\multicolumn{4}{|c|}{Anchored A}\\
\hline
Partial matrix-loading &  
    \begin{minipage}{.1\textwidth}
  \includegraphics[scale=0.6]{Figures/matrix_partials.pdf}
    \end{minipage} &
    
  $\frac{W}{W'};\frac{C}{C'};\frac{H}{H'}$  &
    \begin{minipage}{.1\textwidth}
      \includegraphics[scale=0.6]{Figures/step_line_multi.pdf}
    \end{minipage}    \\




%Partial matrix-loading &  
%    \begin{minipage}{.1\textwidth}
%  \includegraphics[scale=0.6]{Figures/matrix_partials.pdf}
%    \end{minipage} &
%    \multirowcell{1}{
%   $\frac{C}{C'};\frac{(P.K)} {(P' .K')};1$ \\ \\$\frac{C}{C'},\frac{(P \times K)}{(P' \times K')};$ \\$\frac{C}{C'}$} &
%   \multirowcell{1}{ \begin{minipage}{.1\textwidth}
%      \includegraphics[scale=0.6]{Figures/step_line.pdf}
%    \end{minipage} \\ (B along col.) \\  \begin{minipage}{.1\textwidth}
%      \includegraphics[scale=0.6]{Figures/step_line_multi.pdf}
%    \end{minipage} \\ (B along row)}    \\

& & & \\
%& & & \\
%& & & \\
%& & & \\
%& & & \\
%& & & \\

\hline
\rowcolor{blue!10}
\multicolumn{4}{|c|}{Anchored B}\\
\hline

Partial matrix-loading &  
    \begin{minipage}{.1\textwidth}
  \includegraphics[scale=0.6]{Figures/matrix_partials.pdf}
    \end{minipage} &
   $\frac{H} {H'};\frac{C}{C'} ;\frac{W}{W'} $ &
    \begin{minipage}{.1\textwidth}
      \includegraphics[scale=0.6]{Figures/step_line_multi.pdf}
    \end{minipage}   \\








%Partial matrix-loading &  
%    \begin{minipage}{.1\textwidth}
%  \includegraphics[scale=0.6]{Figures/matrix_partials.pdf}
%    \end{minipage} &
%  \multirowcell{1}{ $\frac{C}{C'} ; \frac{(P \times K)} {(P' \times K')};1 $\\ \\ \\
%  $\frac{C}{C'}; 1; \frac{(P\times K)}{(P' \times K')}$} &
%   \multirowcell{1}{ \begin{minipage}{.1\textwidth}
%      \includegraphics[scale=0.6]{Figures/step_line.pdf}
%    \end{minipage} \\ (A along row) \\  \begin{minipage}{.1\textwidth}
%      \includegraphics[scale=0.4]{Figures/sawtooth.pdf}
%    \end{minipage} \\ (A along col.}    \\

%& & & \\
%& & & \\
%& & & \\
%& & & \\
%& & & \\
& & & \\

\hline

\hline
\rowcolor{blue!10}
\multicolumn{4}{|c|}{Anchored Output}\\
\hline
Partial matrix-loading &  
    \begin{minipage}{.1\textwidth}
  \includegraphics[scale=0.6]{Figures/matrix_partials.pdf}
    \end{minipage} &
   $ \frac{(H \times W)} {(H' \times W')} ;\frac{C}{C'} ;1$ &
    \begin{minipage}{.1\textwidth}
      \includegraphics[scale=0.4]{Figures/sawtooth.pdf}
    \end{minipage}   \\



\hline
\hline

%Column-major loading  &  
%%    \begin{minipage}{.1\textwidth}
%      \includegraphics[scale=0.5]{Figures/matrix_full.pdf}
%    \end{minipage} & $C' ; 1 $ &  \begin{minipage}{.1\textwidth}
%      \includegraphics[scale=0.5]{Figures/line.pdf}
%    \end{minipage} \\
%\hline
%\hline


Row-major loading  &  
    \begin{minipage}{.1\textwidth}
      \includegraphics[scale=0.6]{Figures/row_major.pdf}
    \end{minipage} & $ \frac{H\times W} { H' \times W'};1;1 $ &  \begin{minipage}{.1\textwidth}
      \includegraphics[scale=0.3]{Figures/straight.pdf}
    \end{minipage} \\
\hline
\hline

No tiling & 
    \begin{minipage}{.1\textwidth}
      \includegraphics[scale=0.5]{Figures/matrix_full.pdf}
    \end{minipage} &   $1;1;1$ &  \begin{minipage}{.1\textwidth}
      \includegraphics[scale=0.1]{Figures/circle.pdf}
    \end{minipage} \\
\hline
\end{tabular}
\caption{\label{tab:dataflow_matrix} Pattern Table for Matrix multiplication: Various possibilities for tiling the input (H', C', W' represents the tiling factor, different colors represent various output tiles.}
\end{center}
\end{table}
\end{scriptsize}


%\subsubsection{Doubly circulant matrix: Converting convolution to a classical matrix multiplication problem}
%A 2D convolution can be computed using a \textit{doubly block circulant matrix}. In this scheme, the rows of the matrix $B$ are generated by flattening the input of size $P \times Q$, which will create a column matrix of dimension $P.Q \times 1$. A weight matrix of dimension $R\times S$ generates the doubly block circulant matrix. We compute the first row of size $P.Q$ by flattening the complete weight matrix. The zeros are added in the row, as required. We generate the subsequent rows by shifting the previous row. The method transforms the whole convolution into a simple matrix multiplication. 













==> architecture.tex <==
\section{Architecture}
\subsection{Overview}

\subsection{Crypto-engine}


==> newintro.tex <==
\section{Introduction}

The AI hardware market was valued at 8 billion USD in 2020 and is expected to grow to 
84 billion USD by 2028~\cite{verifiedmarketresearch} (CAGR of 34.15\%). Hardware-based
AI chips are expected to play a major role in telecommunications~\cite{}, mobile
vision~\cite{}, and edge computing~\cite{}. augmented/virtual reality~\cite{}, 
healthcare~\cite{}, and autonomous driving~\cite{}. Similar to code for general-purpose
processors, ML models
incorporate a lot of high-value intellectual property (IP) that takes a lot of time and
effort to collate and develop. For example, even for a mid-size AI project just collecting
the raw data using mechanical turks takes upwards of \$100K USD~\cite{}; the know-how 
for the model and training methodology can be worth millions of dollars, and finally 
it may take many weeks to finally train the model using large cluster computers.
Along with these conventional arguments, many a time we don't realize that even getting access
to the training data can be quite challenging with numerous legal hurdles. 
Hence, we can conclude that protecting an ML model is of paramount importance, and also 
it is an attractive target for hackers to steal. 

There are three broad approaches for protecting models as shown in Figure~\ref{}. All of them
rely on secure CPUs as the baseline technology. To secure CPUs, we use Trusted Execution 
Environments (TEEs) such as Intel SGX~\cite{}, AMD SEV~\cite{}, and ARM Trustzone~\cite{}.
In all these TEEs, the CPU is assumed to be secure; it is within the {\em TCB} (Trusted 
Computing Base). The main contribution of the most elaborate scheme, Intel SGX, 
is in protecting the off-chip memory and providing
confidentiality, integrity, and freshness. The key insight is ensuring that every time 
a block is written to main memory, it is encrypted with a different key. Since, storing
a key for every memory block is too expensive, a more efficient mechanism is used based on
AES counter-mode encryption. Every page is associated with a major counter, and every block
uses a minor counter (a combination of both guides the encryption/decryption). The counters
themselves need to be protected; this is achieved using a Merkle tree, where the root of 
the tree is guaranteed to be in the TCB.  Let us refer to this version of SGX as {\em SGX-Client}.
Because of the Merkle tree and associated overheads of maintaining counters, the maximum 
size of the protected memory region is limited to 128-256 MB (same problem with
ARM TrustZone). Most ML models and datasets
as of today  are much larger. As a result, {\em SGX-Client} is not the best choice for them.

Keeping in mind these issues, Intel recently discontinued support for {\em SGX-Client} in its
$11^{th}$ and $12^{th}$ generation processors. It replaced it with another version of SGX 
(referred to as {\em SGX-Server}) that simply encrypts memory and foregoes the integrity and
freshness guarantees~\cite{} (on the lines of AMD SEV). It can provide up to 512 GB of encrypted
memory. We should bear in mind that {\em SGX-Server} is far weaker than {\em SGX-Client} in
terms of the security guarantees that are provided namely integrity and freshness.

ML architecture designers have traditionally opted to use versions of {\em SGX-Client} to secure
their systems (refer to Figure~\ref{}). Several early approaches either proposed optimizations
to {\em SGX-Client}~\cite{} to reduce its overhead or partition an ML algorithm into a secure portion
and unsecure portion that ran on fast hardware such as GPUs~\cite{}. However, these approaches have
been superseded by a newer family of approaches that leverage the stable data communication
patterns of ML workloads to design bespoke NoCs. Two custom accelerators stand out in this space: 
TNPU~\cite{} and GuardNN~\cite{}. Their basic ideas are similar: group a set of contiguous memory
blocks into {\em tiles} and provide freshness guarantees at the level of a tile. Both use a dedicated
scheduler that runs on the host CPU (using a TEE similar to {\em SGX-Client}) for scheduling
and managing version numbers (VNs), which are used to encrypt data as well as ensure its freshness. 
The major difference is that TNPU stores the VNs in an on-chip cache and
GuardNN relies on a CPU program to generate all the VNs. The program needs to store all the VNs
in use in secure memory, and securely communicate them to the accelerator (a difficult problem
in itself).
Both still perform integrity checking at the 
level of individual memory blocks (typically 64 bytes).

Our scheme, \fname, improves upon these ideas and proposes a natural extension, where we 
perform freshness and integrity checks at
\underline{the tile level}. Given that no data is stored or computation is done at the block-level 
(like previous schemes), there is an associated performance gain (XX-XX\%). Additionally, there is
no need to run a dedicated scheduler in the host CPU with a TEE  like {\em SGX-Client}. 
This is achieved as follows.
We thoroughly characterize the memory access patterns of different kinds of ML accelerators, efficiently
encode them, and pass them to a small hardware circuit that automatically generates all VNs
(without external intervention). This eliminates the need for storing and managing VNs in on-chip 
caches or main memory regions.

To summarize, {\bf the main contributions in this paper} are as follows: (1) Characterization of traffic in 
CNNs and popular data pre/post processing algorithms, (2) A method to succinctly encode the traffic pattern,
(3) A method to generate VNs on the fly using such patterns, (4) A technique to
 perform integrity checking at the level of tiles, and (5) A detailed experimental analysis of \fname that
shows a XX-XX\% speedup over the nearest competing work. (6) Given that the overheads are low, we additionally
assess the benefits of interspersing the execution with the running of a dummy network (for the purpose of
adding noise). This helps reduce the possibility of model extraction attacks by utilizing timing or address
side channels substantially.


The paper is organized as follows.
Section~\ref{sec:background} presents the background of TEEs and basic convolution
operations in neural networks. Section~\ref{sec:ThreatModel} presents the threat model and the 
security guarantees provided by \fname.
We characterize the workloads in Section~\ref{sec:characterization}, 
present an analytical model for automatic version number generation in   Section~\ref{sec:PatternAnalysis}, and
present the architecture of \fname in 
Section \ref{sec:architecture}. Finally, Section \ref{sec:results} reports the
experimental results, Section~\ref{sec:RelatedWork} presents the related work and we conclude in Section
\ref{sec:conclusion}.













